Differentiable Artificial Reverberation

Artificial reverberation (AR) models play a central role in various audio applications. Therefore, estimating the AR model parameters (ARPs) of a reference reverberation is a crucial task. Although a few recent deep-learning-based approaches have shown promising performance, their non-end-to-end training scheme prevents them from fully exploiting the potential of deep neural networks. This motivates the introduction of differentiable artificial reverberation (DAR) models, allowing loss gradients to be back-propagated end-to-end. However, implementing the AR models with their difference equations "as is" in the deep learning framework severely bottlenecks the training speed when executed with a parallel processor like GPU due to their infinite impulse response (IIR) components. We tackle this problem by replacing the IIR filters with finite impulse response (FIR) approximations with the frequency-sampling method. Using this technique, we implement three DAR models -- differentiable Filtered Velvet Noise (FVN), Advanced Filtered Velvet Noise (AFVN), and Delay Network (DN). For each AR model, we train its ARP estimation networks for analysis-synthesis (RIR-to-ARP) and blind estimation (reverberant-speech-to-ARP) task in an end-to-end manner with its DAR model counterpart. Experiment results show that the proposed method achieves consistent performance improvement over the non-end-to-end approaches in both objective metrics and subjective listening test results.

==> figures/ablations.tex <==
\begin{figure}[t]
    \begin{center}
        \centerline{\includegraphics[width=\columnwidth]{figures/pdfs/ablations.pdf}}
        \caption{BLABLABLA.}
        \label{fig:fdn-model}
    \end{center}
\end{figure}
    
    


==> figures/edr_plot.tex <==
\begin{figure}[]
    \begin{center}
        \centerline{\includegraphics[width=.98\columnwidth]{figures/pdfs/bulkbulk22.pdf}}
        \caption{EDR contour plots of the ground-truth RIRs and their estimations with the trained networks. The $x$- and $y$-axis denote frequency ($\si{Hz}$) and time ($\si{s}$). Plots on the same column show the same ground truth (blue curves). Each network's estimations with the DAR, AR models (red curves with different line styles) are drawn for each target. The $0\si{dB}$, $-20\si{dB}$, $-40\si{dB}$ and $-60\si{dB}$ contours are drawn, using from the darkest to the brightest colors. 
        }    
        \label{fig:edr}
    \end{center}
    %\vskip -0.2in
\end{figure}

==> figures/fsm-results.tex <==
\begin{figure}[t]
    \begin{center}
        \centerline{\includegraphics[width=.86\columnwidth]{figures/pdfs/fsm-result.pdf}}
        \caption{BLABLABLA.}
        \label{fig:fdn-model}
    \end{center}
\end{figure}
    
    


==> figures/mushra_results.tex <==
\begin{figure}[t]
    \begin{center}
        \centerline{\includegraphics[width=\columnwidth]{figures/pdfs/mushra-2.pdf}}
        \caption{MUSHRA subjective listening test results. }
        \label{fig:mushra}
    \end{center}
\end{figure}
    
    


==> sections/biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/pdfs/shlee-2.png}}]{Sungho Lee} received the BSc degree in Creative IT Engineering from Pohang University of Science and Technology, Republic of Korea, in 2020. He
is currently working towards a Ph.D degree in digital contents and information studies at the Music and Audio Research Group, Seoul National University, Republic of Korea. His research interests include deep learning methods for audio effects and speech enhancement. 

\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/pdfs/hschoi.JPG}}]{Hyeong-Seok Choi}
received the BSc degree in Automotive Engineering from Hanyang University, Republic of Korea, in 2016. He received the Ph.D degree in the Digital Contents and Information Studies at the Music and Audio Research Group, Seoul National University, Republic of Korea, in 2022. He is currently a researcher at the Institute of New Media and Communications, Seoul National University. His research interests include speech enhancement, generative models for audio signal, and self-supervised representation learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/pdfs/kglee.png}}]{Kyogu Lee} received his Ph.D degree in computer-based music theory and acoustics from Stanford University. He is a professor in the Department of Intelligence and Information at Seoul National University and leads the Music and Audio Research Group. His research focuses on signal processing and machine learning techniques applied to music, audio and hearing.
\end{IEEEbiography}
